JUNO: Optimizing High-Dimensional Approximate Nearest Neighbour Search with Sparsity-Aware Algorithm and Ray-Tracing Core Mapping

Approximate nearest neighbor (ANN) search is a widely applied technique in modern intelligent applications, such as recommendation systems and vector databases. Therefore, efficient and high-throughput execution of ANN search has become increasingly important. In this paper, we first characterize the state-of-the-art product quantization-based method of ANN search and identify a significant source of inefficiency in the form of unnecessary pairwise distance calculations and accumulations. To improve efficiency, we propose JUNO, an end-to-end ANN search system that adopts a carefully designed sparsity- and locality-aware search algorithm. We also present an efficient hardware mapping that utilizes ray tracing cores in modern GPUs with pipelined execution on tensor cores to execute our sparsity-aware ANN search algorithm. Our evaluations on four datasets ranging in size from 1 to 100 million search points demonstrate 2.2x-8.5x improvements in search throughput. Moreover, our algorithmic enhancements alone achieve a maximal 2.6x improvement on the hardware without the acceleration of the RT core.

==> discussions.tex <==

\section{Further Discussions}
\label{sec:discussion}
In this section, we further discuss some strongness related topics in the process of \proj{} studying.
\paragraph{Accuracy Guarantee}
\paragraph{\proj{}'s Benefits and Nature of Datasets}

==> methodology.tex <==
% \section{\proj{} Design and Implementation}
%\section{Threshold Based Selective L2-LUT Construction and RT Core Mapping}
\section{Selective L2-LUT Construction on RT Core}
% In this section, we present our algorithm-software co-designed framework called \proj{} that exploits the aforementioned sparsity and spatial locality in the codebook entries to achieve the high-performance ANN search in high-dimensional spaces.
% We begin by introducing our algorithmic intuition that enables the utilization of RT core for high-dimensional ANN search. 
% Next, we provide a comprehensive description of the methodology employed in \proj{} from both algorithmic enhancement and hardware mapping perspectives. Finally, we discuss optimizations and trade-offs associated with our framework.
 
%\proj{} is an algorithm-hardware mapping co-design to enable high performance ANN search in high dimensional space.
%In this section, we first describe the intuition of applying RT hardware to leverage sparsity and spatial locality mentioned in \Sec{sec:Motivation} to accelerate ANN search in high dimensional space. We then precisely describe the methodology of \proj{} from algorithm enhancement and hardware mapping aspects. Finally we discuss some optimizations and trade-offs.  

In this section, we present our algorithm enhancement and RT core mapping for an efficient alternative of orignial \emph{L2-LUT construction} stage.
We begin by introducing our algorithmic intuition and design details, then we introduce how we map the enhanced algorithm to the RT core. 

\subsection{Threshold Based Selective L2-LUT Construction}
\label{sec:ThresholdBasedL2LUT}
In this subsection, we describe and explain our algorithm design to leverage the aforementioned features of current ANN search. The new algorithm aims to replace current \emph{L2-LUT construction} in our searching pipeline, and provide significant operation saving with acceptable approximation.

\paragraph{Intuition of Algorithm Enhancement.}
\label{sec:Intuition}
% 1. We mainly use a threshold based distance check to rapidly filter out the points we are not insterested in
% 2. With this distance threshold we can save a lot of computationcalculation with cheaper AABB intersection check.
% To leverage the sparsity and spatial similarity in codebook entries usage in typical \texttt{IVFPQ} process as mentioned in \Sec{sec:Motivation}, we design a distance checking based method to replace \emph{L2-LUT construction} stage, which can rapidly filter in the search points with higher probability to be the nearest neighbours. 
% To be specific, we set distance thresholds in all subspaces, we then define the interested region of a query projection as the union of all points with distance from the query projection being less than the distance threshold.  
% We abandon codebook entries fall outside the interested region of a query projection. Only search points whose codebook entries fall inside the interested region are preserved for later \emph{distance calculation} stage. This is reasonable because the actually used codebook entries are closely distributed around the query projection according to the finding in \Sec{sec:Motivation}.

Our algorithm aims to exploit the sparsity and spatial locality in subspaces, resulting in improved search performance through additional approximation techniques alongside product quantization. 
Specifically, we propose a distance checking-based approach to efficiently prune unnecessary entries in each subspace. This approach involves setting distance thresholds in all subspaces, defining the interested region of a query projection as the union of all points with distances from the query projection being less than the distance threshold, and subsequently discarding codebook entries that fall outside the interested region of a query projection. This pruning strategy is motivated by the findings presented in \Sec{sec:Motivation}.

%Our algorithm focuses on leveraging the sparsity and spatial locality in subspaces, and improve the search performance by doing more approximation in these subspaces besides quantization. 
%We design a distance checking based method to prune the unnecessary entries in every subspace. To be specific, we set distance thresholds in all subspaces, we then define the interested region of a query projection as the union of all points with distance from the query projection being less than the distance threshold. We then abandon codebook entries fall outside the interested region of a query projection, based on the finding of \Sec{sec:Motivation}.

\begin{floatingfigure}{4.5cm}
    \centering
    \includegraphics[width=0.5\linewidth]{SaveOp.pdf}
    \caption{Remained search points that need to calculate the distance when changing threshold.}
    \label{fig-SaveOp} 
\end{floatingfigure}
Pruning unnecessary codebook entries can significantly reduce the number of distance calculations. As depicted in \Fig{fig-SaveOp}, the remaining search point projections that require looking up the L2-LUT and distance calculations decrease linearly with the threshold. This finding suggests that the projections of the top-100 search points are closely distributed around the query projection in a subspace. Consequently, a substantial amount of L2-LUT lookups and distance calculations can potentially be saved by filtering out codebook entries that are far away from the query projection in each subspace.

%By pruning unnecessary codebook entries, a large amount of distance calculations can be reduced. As shown in \Fig{fig-SaveOpAndTwoMethod}(a), the remained search point projections that need to look up the L2-LUT and do distance calculation decrease linearly with the threshold. Given the finding that projection of top-100 search points are closely distributed around the query projection in a subspace, potentially we can save huge amount of L2-LUT looking up and distance calculation after filtering out the codebook entries being far away from the query projection in every subspace.


% Our method relies on the inside/outside check in low dimension Euclidean subspace.
% This matches the RT core very well since the RT core is hardware that can efficiently check intersecting or not in Euclidean space, and the inside/outside check can be easily transformed to intersection test.
% Moreover, the RT core check the intersection of spatially close objects on a sparse friendly data structure (tree-based bounding box searching), which is significantly affinitive to the features we find in \Sec{sec:Motivation}, that used codebook entries in \texttt{IVFPQ} is sparse while closely distributed in the euclidean space. 

% Prior work~\cite{RTNN} has shown that the RT core is capable of efficiently conducting inside/outside checks without having to calculate all pairwise distances, thanks to its BVH tree-based algorithm. 
% By leveraging this capability, our method can potentially save computational resources in determining whether an entry falls inside the region of interest within a query projection in a subspace. To achieve this, we map our distance-checking approach to the RT core by placing a sphere at the coordinates of the query projection, with a radius set to the distance threshold. This sphere naturally defines the region of interest. Subsequently, we can shoot rays from codebook entries towards the region of interest in the RT core to quickly determine if an entry falls within the region of interest.

%According to the previous work~\cite{RTNN}, the RT core can conduct efficient inside/outside check without calculating all pairwise distance thanks to its BVH tree based algorithm. So we can save more distance calculation in determining whether or not an entry falls inside the interested region of a query projection in a subspace, if we map our distance checking based method to the RT core. 
%Thus, we map our method to the RT core by placing a sphere at the coordinate of the query projection, with the radius set to the distance threshold, this sphere is naturally the interested region. Then we can shoot rays from codebook entries towards the interested region to quickly check if a entry falls into the interested region with the RT core. 
% \begin{figure}[t]
%       \includegraphics[width=0.99\linewidth]{SaveOp.pdf}
%     \caption{Remained search points that need to calculate the distance when changing threshold.}
%     \label{fig-SaveOpAndTwoMethod} 
% \end{figure}


% In addition, performing only the intersection test, as opposed to the exact distance calculation on the RT core, is more cost-effective and also faster. 
% As a result, we can employ a more aggressive approximation, wherein only the count of search points falling inside the interested region of a query projection in each subspace is recorded, thereby eliminating the need for all distance calculations. This approximation is supported by previous research~\cite{?}, which has found that as the number of subspaces in which the search point projection is close to the query projection increases, so does the probability that the search point is close to the query in the original space.

%Moreover, it is much cheaper and faster to do the intersection test only than exact distance calculation on the RT core. 
%Thus, we can do a more aggressive approximation that can save all distance calculations by only recording the count of a search point that falls inside the interested region of a query projection in every subspace.
%This approximation is supported by previous work's finding that in more subspaces the search point projection being close to the query projection, the higher the probability the search point is close to the query in the original space. 

% Different applications have different performance and search quality requirement. With our distance checking based method and RT core mapping, we can do a even more aggressive approximatation that can save all distance calculation by only recording the times of a search points falls inside the interested region of query projection in all subspaces. Moreover, the intersection test only is much cheaper and faster than exact distance calculation. According to previous work, with enough pairwise inside/outside comparisons between search point projections and query's interested region in subspaces, we have high probability to reach the nearest neighbour combining the inside/outside results from all subspaces~\cite{NNHighDim} . 

\paragraph{Choose Necessary Entries with Efficiency.}
As discussed in \Sec{sec:Intuition}, our algorithm leverages the sparsity and spatial locality by selectively choosing the codebook entries that fall within the region of interest in each subspace. 
The distances between these selected entries and the query projection are then calculated for constructing a \emph{L2-LUT} in a selective manner. To achieve this, we bound smaller entries/boxes into a larger box and hierarchically organize these bounding boxes into a tree structure. As such, we can avoid pairwise distance calculations between all $E$ entries and the query projection in each subspace, and instead perform inside/outside checks with logarithmic complexity of $logE$.

%As mentioned in \Sec{sec:Intuition}, our algorithm leverages the sparsity and spatial locality by only selecting the codebook entries fall inside the interested region of the query projection in a subspace, and calculate their distance for a selective \emph{L2-LUT construction}. By bounding an entry/smaller boxes into a box and hierarchically organize these bounding boxes into a tree, we can avoid pairwise distance calculation between all $E$ entries and query projection in every subspace, and conduct the inside/outside check with $logE$ scale complexity.

\paragraph{Determining Proper Threshold.}
The selection of an appropriate threshold is crucial in our approach, as it is used to distinguish whether an entry falls within the interested region of a query projection. A tight threshold may filter out too many entries, resulting in missed true neighbors, while a relaxed threshold may include unnecessary entries, leading to wastage of time and resources. To determine the optimal threshold, we conduct a thorough study on the relationship between query features and the threshold that can contain the top-100 search points in each subspace.
 
%Recall that we rely on a threshold to distinguish whether or not an entry falls inside a interested region of a query projection. To choose a proper threshold is critical. A tight threshold may filter out too much entries thus miss some true neighbour, while a relax threshold may include unnecessary entries, resulting in time and resource wastage. To determine a proper threshold, we first study the relation between query features and threshold that can contain top-100 search points on every subspace. 

\begin{figure}[t]
    \centering
      \includegraphics[width=0.485\linewidth]{RadiusDensity.pdf}
      \includegraphics[width=0.49\linewidth]{RadiusPowerPattern.pdf}
    \caption{(a) The relation between threshold to contain top-100 search points and region density a query falls into. (b) The amount of top-100 search points contained when threshold scales smaller. }
    \label{fig-radius} 
\end{figure}

As shown in \Fig{fig-radius}(a), we observe a negative correlation between the threshold for containing the top-100 search points and the region density of the query projection in a subspace. To calculate the region density, we divide the entire subspace into a $100 \times 100$ grid and define the density of each cell as the quotient obtained by dividing the number of search point projections falling into that cell by the area of the cell. This finding is reasonable, as a higher threshold is likely to contain many search point projections in high-density regions, resulting in a higher probability of containing the top-100 search points. Conversely, in low-density regions, even the same threshold may not be able to contain 100 search point projections, let alone the top-100 points.

%As shown in \Fig{fig-radius}(a), we find that threshold to contain top-100 search points has negative correlation to the region density the query projection locates in a subspace. To calculate the region density, we divide the whole subspace into $100\times 100$ grid, and define the density of one cell as quotient of dividing amount of search point projection fall into this cell by the area of this cell. 
%This finding is reasonable since a threshold may contain many search point projection in high density region, thus the probability of containing top-100 search points is high. While in low density region, a same threshold even can not contain 100 search points projection, not to say top-100 points. 

Based on our findings, we propose incorporating dynamic radius mechanics to determine an appropriate threshold during runtime. Initially, we generate a density map and a simple regression model offline. The density map consists of a $100\times 100$ grid for each subspace, where each cell records the density computed as previously described. Subsequently, we randomly select several search points projections to train the regression model, with the region density as input and the threshold to contain the top-100 search points as output. During runtime, we lookup the density of the query projection in each subspace and use the regression model to infer a query-specific threshold. Notably, we find that a simple polynomial regression model accurately captures the relationship, resulting in minimal runtime overhead for threshold determination. Once the threshold is determined, we disregard all codebook entries beyond the threshold and compute the distance between the query projection and the remaining codebook entries to create an L2 lookup table (L2-LUT).

%Based on this finding, we introduce dynamic radius mechanics to choose the proper threshold at runtime. First, we prepare a density map and a simple regression model offline. The density map is a $100\times 100$ grid for every subspace, with each cell recording the density calculated as mentioned before. We then randomly sample several search points projection to train the regression model with the region density they locate as input and threshold to contain top-100 search points as output. At runtime, we lookup the density of query projection in every subspace and inference the regression model for a query-specific threshold. Notice that we find a simple polynomial regression model fits the relation well, so the runtime overhead of determining proper threshold is low. Once determining the threshold, we ignore all codebook entries beyond the threshold and calculate the distance between query projection and remained codebook entries for a L2 lookup table.

Furthermore, we have observed a power-law pattern in the variation of the threshold value, as illustrated in \Fig{fig-radius}(b). When the distance threshold is scaled down to half of its original value to accommodate the top-100 search points, approximately 90\% of these points are retained. This indicates the potential for using a smaller distance threshold to further prune codebook entries. In other words, we can trade-off slightly lower search quality for significantly enhanced search throughput, such as queries per second (QPS). In our work, we provide users with the flexibility to set the threshold value through a dedicated interface, enabling them to make this trade-off according to their specific needs.

%Furthermore, we have observed a power-law pattern when varying the threshold value. As depicted in \Fig{fig-radius}(b), when the distance threshold is scaled down to half of its original value in order to accommodate the top-100 search points, around 90\% of these points are still retained. 
%This indicates the opportunity of using a smaller distance threshold to prune even more codebook entries.
%In other words, we can trade-off a slightly lower search quality for a much more enhanced search throughput (e.g., query per second or QPS).
%In our work, we offer this trade-off flexibility and provide users the ability to set the threshold value through a dedicated interface.


%Besides, we observe power pattern when trying different threshold. As shown in \Fig{fig-radius}(b), if we scale the threshold to half of the threshold to contain top-100 search points, still around 90\% of the top-100 are contained. But with smaller threshold, less entries will be used, leading to higher sparsity thus higher chance to save resources. In scenarios with low search quality requirement, a smaller threshold can be set for higher QPS. In contrast, users can also set bigger threshold to consider at most all codebook entries for extremely high search quality. We leave this option to the users by providing a threshold setting interface.

\subsection{Mapping the Selective Algorithm to the RT Core}

In this subsection, we explain how to map the computation of selective L2-LUT construction described in \Sec{sec:ThresholdBasedL2LUT} to the ray-tracing (RT) core in modern GPUs.
The RT core implements bounding box intersection check (AABB) and hierarchical data structure traversing (BVH) in the hardware, which aligns with the computational characteristics of our proposed threshold-based LUT construction.
Similar to the original ANN search algorithm discussed in \Sec{subsec:ann_background}, our RT-core-based ANN algorithm comprises of both an offline and online component.
Furthermore, we provide technical details on how to enable dynamic thresholding, calculate distance, and support inner (or dot) product metric.
%We also describe the technical details about how to enable dynamic threshold, how to calculate distance and enable inner (or dot) product metric.

{
\begin{algorithm}[b]
\small
	\caption{Build a traversable scene, prepare cluster centroids of filter and entry-search points mapping offline.}
	\label{Algo-BuildIndex}
	\textbf{Input:}  $points\lbrack N\rbrack \lbrack D \rbrack$, $M=2$, $E$, $C$, $metric$\\
    \textbf{Output:} $Map\lbrack C\rbrack\lbrack \frac{D}{M}\rbrack\lbrace entry\_id : points\_id\lbrack~\rbrack  \rbrace$\\
    \textbf{Output:} $centroids, labels$\\
    \textbf{Output:} $Traversable\_Scene$
	\begin{algorithmic}[1]
		\Function {BuildRTScene}{$points\lbrack N\rbrack \lbrack D \rbrack$, $M$, $E$, $C$}
        \State{$Traversable\_Scene\leftarrow \emptyset$}
        \State{$filter\leftarrow kmeans(points, n\_cluster=C)$}
        \State{$centroids, labels\leftarrow filter.centroids, filter.labels$}
        \State{$residual\leftarrow\lbrack x-centoids\lbrack x.label\rbrack for~x~in~points\rbrack$}
        \For{$s\in\lbrack 0, \frac{D}{M})$}
            \State{$res\leftarrow residual\lbrack:,2s:2s+2\rbrack$}
            \State{$codebook[s]\leftarrow kmeans(res, n\_cluster=E)$}
            \State{$entries\leftarrow codebook[s].centroids$}
            \For{$e\in[0,E)$}
                \State{$x,y,z\leftarrow entries[e].x,entries[e].y,2s+1$}
                \State{$threshold\leftarrow PolyRegression(density_{(x,y)})$}
                \State{$sphere\leftarrow(center=(x,y,z),r=threshold)$}
                \State{$Traversable\_Scene.add(sphere)$}
            \EndFor
            \For{$e\in\lbrack 0, E),c\in\lbrack 0, C)$}
                \State{$res_{c}\leftarrow \lbrack labels[p]=c~for~p~in~res \rbrack$}
                \State{$Map\lbrack c \rbrack\lbrack e\rbrack\leftarrow \lbrack  p~encoded~by~e~for~p~in~res_{c}\rbrack$}
            \EndFor
        \EndFor
        \State{\textbf{return }$Traversable\_Scene, Map, centroids, labels$}
		\EndFunction
	\end{algorithmic}
\end{algorithm}
}

\paragraph{Intuition of Hardware Mapping.}
\begin{figure}[t]
    \centering
      \includegraphics[width=0.99\linewidth]{JUNOIntuition.pdf}
    \caption{Intuition of hardware mapping of \proj{}.}
    \label{fig-Intuition} 
\end{figure}
Prior work~\cite{RTNN} has shown that the RT core is capable of efficiently conducting inside/outside checks without having to calculate all pairwise distances, thanks to its BVH tree-based algorithm. 
By leveraging this capability, our method can potentially save computational resources in determining whether an entry falls inside the region of interest within a query projection in a subspace. To achieve this, we map our distance-checking approach to the RT core by placing a sphere at the coordinates of the query projection, with a radius set to the distance threshold. This sphere naturally defines the region of interest. Subsequently, we can shoot rays from codebook entries towards the region of interest in the RT core to quickly determine if an entry falls within the region of interest, as shown in the left part of \Fig{fig-Intuition}. 

After obtaining the entries within the region of interest, we calculate the hit distance representing the exact distance from an entry to a query projection in a subspace to generate a L2-LUT for further distance calculation using. Naively we need to lookup for hit entries' coordinates, while with hit time $t$ returned by the RT core, we are free from any lookup when calculate hit distance. Once the L2-LUT is constructed, we can conduct further distance lookup and calculation for the interested search points as shown in the right part of \Fig{fig-Intuition}.

In addition, performing only the intersection test, as opposed to the exact distance calculation on the RT core, is more cost-effective and also faster. 
As a result, we can employ a more aggressive approximation, wherein only the count of search points falling inside the interested region of a query projection in each subspace is recorded, thereby eliminating the need for all distance calculations. This approximation is supported by previous research~\cite{?}, which has found that as the number of subspaces in which the search point projection is close to the query projection increases, so does the probability that the search point is close to the query in the original space.

\paragraph{Offline.} 
In offline stage we need to prepare a traversable scene and a subspace level inverted indices for later online searching. We follow the typical \texttt{IVFPQ} offline training process to first obtain the $C$ cluster centriods and labels of search points needed by \emph{filter} stage (line 3-4 of \Alg{Algo-BuildIndex}), and second obtain the codebook trained by the residual between search points and their centroids, (line 5-9 of \Alg{Algo-BuildIndex}). However, in contrast to typical \texttt{IVFPQ} encodes and stores all search points with the codebook entries, we maintain a inverted index from codebook entries to search points (line 14-16 of \Alg{Algo-BuildIndex}) in every subspace, the $Map[114][19][24]$ contain all search points satisfying followings condition: i) the search point belongs to $114^{th}$ cluster, ii) the projection of the search point is encoded with $24^{th}$ codebook entry in $19^{th}$ subspace. This inverted index enables us to only iterate necessary search points from entries being close to the query projection in a subspace. 

% Our main idea of mapping the algorithm to the RT core is to let the RT core check whether or not an codebook entry falls inside the interested region of a query projection controlled by a threshold. 
Intuitively we use a sphere to mark the interested region of a query projection, while this requires adding spheres into the RT scene at runtime, which has unacceptable overhead. Thanks to the commutativity of the L2 distance, we can create spheres at the location of codebook entries offline, so that when a ray representing query projection is shot towards these sphers, it can get identical inside/outside result too. 
For the $d^{th}$ subspace, we put the spheres representing entries of this subspace at entries' $x$ and $y$ coordinates. For $z$, we place the entries from different subspace at different depth, i.e. $z=2s+1$ for $s^{th}$ subspace, to avoid interfered by rays from other subspaces when doing ray tracing. Line 10-13 of \Alg{Algo-BuildIndex} shows the placement of codebook entries in $D/M$ subspaces, this is also demostrated in the left part of \Fig{fig-Intuition}. 

After determining the position of spheres, we need to determine the radius representing the threshold. Notice that the threshold depend on the region density a query projection falls into, and we can set every sphere a radius to be this threshold, and this threshold is now calculated using region density of the codebook entry instead of the query projection. For now, this method is unable to support user-defined threshold scaling factor and QPS/quality trade-off since the overhead of building a traversable scene online is unacceptable, and we will introduce hit time based method to enable this feature in \Sec{sec:HitTime}.

\paragraph{Online.} 
\label{sec:Online}
We first describe the situation of a single query, and this is straightforward to generalize to the multi-query situation. Since the codebook entries are trained with residuals, we need to calculate the residual between query and centroids of its selected clusters too (line 4-5 of \Alg{Algo-L2LUT}). For every selected cluster, we create a ray starting from the coordinate of residual between query projection and cluster centroid projection in every subspace (line 6-7 of \Alg{Algo-L2LUT}). Recalling that we put the spheres representing codebook entries in $s^{th}$ subspace at $z=2s+1$, if we place the ray origin at $z=2s$ and let the $t_{max}$ of rays to be $1.0$, these rays can correctly interact with the spheres in the same subspace as we expect without interfering entries in other subspaces, as shown in the left part of \Fig{fig-Intuition}. 

Obviously, only when an entry falls into the interested region of a query projection in a subspace will the ray hit the sphere thus call the hit shader. Once a hit event occurs, we calculate and record the the actual distance between the entry and the query projection with $t_{hit}$. We create and shoot rays of all projections of all queries in parallel, and maintain for every query a list recording the hit entries ID and corresponding distance in every subspace (line 14-16 of \Alg{Algo-L2LUT}).  These lists are the L2 lookup table.

\begin{algorithm}[h]
\small
	\caption{Use the RT core to conduct threshold based selective \emph{L2-LUT construction} online}
	\label{Algo-L2LUT}
    \textbf{Input:} $queries\lbrack Q \rbrack\lbrack D \rbrack$, $index$, $query\_select\_clusters$, $nprobs$\\
    \textbf{Output:} $L2\_LUT[Q][nprobs][\frac{D}{M}]\lbrace entry\_id:distance \rbrace$
	\begin{algorithmic}[1]
		\Function {L2\_LUT}{$query$, $index$, $query\_select\_clusters$}
        \State{$rays\leftarrow\lbrack ~ \rbrack$}
        \For{$q\in\lbrack 0,Q),s\in\lbrack 0, \frac{D}{M})$}
            % \State{$clusters\leftarrow query\_select\_clusters\lbrack q\rbrack$}
            \State{$x,y,z\leftarrow q\lbrack \_q\rbrack\lbrack 2s:2s+1 \rbrack, 2s$}
            \For{$c$\textbf{ in }$query\_select\_clusters[q]$}

                \State{$x,y=(x,y)-index.centroids\lbrack c\rbrack\lbrack 2s:2s+1\rbrack$}
                \State{$rays.add(x,y,z,t_{max}=1,dir=z)$}
            \EndFor
        \EndFor
        \State{$index.scene.set\_hit\_callback($\textbf{RT\_HitShader}$)$}
        \State{\textbf{return }\textbf{RayTracing(}$rays, scene$\textbf{)}}
		\EndFunction
        \Function {RT\_HitShader}{$index$,$query\_select\_clusters$}
        \State{$ray, sphere,t\leftarrow$\textbf{GetRay(),GetHitSphere(),GetTime()}}
        \State{$q,s,e\leftarrow ray.qid, ray.sid, sphere.eid$}
        \State{$distance\leftarrow \sqrt{R^2 - (1-t)^2}$}
        \For{$c$\textbf{ in }$query\_select\_clusters$}
                \State{$L2\_LUT[q][c][s].add(\lbrace e:distance \rbrace)$}
        % \State{$candidate\lbrack ray.qid\rbrack.add(Map_{2^{nd}}\lbrack c\rbrack\lbrack sphere.eid\rbrack)$}
        \EndFor
        \State{\textbf{// Ray continue to find other hit}}
        \EndFunction
	\end{algorithmic}
\end{algorithm}

% \paragraph{Use Max Traverse Time to Enable Dynamic Radius.}
% \label{sec:HitTime}
% As mentioned in \Sec{sec:ThresholdBasedL2LUT}, we can set a radius scaling factor to trade-off between QPS and search quality. We can adjust the $t_{max}$ of rays to control the area rays can hit, thus we avoid changing the radius of spheres at runtime, which has unacceptable overhead. As shown in the right part of \Fig{fig-CalcDistDynR}, with a $t_{max}$ $t$ less than $1.0$, the ray can no longer hit the area with radius greater than $\sqrt{R^{2}-(1-t)^{2}}$. For example, a $t_{max}=0.64$ means a scaling factor to be $0.8$ when the original threshold is $0.6$. We can pass this $t$ as parameter to the ray generation shader, with sevaral floating point arithmetic operation overhead at runtime.

% \paragraph{Supporting Maximal Inner Product Similarity (MIPS).}
% Inner product similarity is widely used in image and word embedding. With some transformation, our methodology can support maximal inner product similarity (MIPS) with almost no cost. Recall that if a query ray hit an entry with radius $R$ at distance $d$ and hit time $t$, we have following relation:
% \begin{equation}
% \label{eq:mips1}
% \begin{aligned}
%     =&1-\sqrt{R^2-d^2}\\=&1-\sqrt{R^2-((x_{e}-x_{q})^2+(y_{e}-y_{q})^2)}\\
%     =&1-\sqrt{R^2-x_{e}^2-y_{e}^2-x_{q}^2-y_{q}^2+2(x_{e}x_{q}+y_{e}y_{q})}
% \end{aligned}
% \end{equation}
% In \Equ{eq:mips1}, $R^2$ and $x_{q}^2,y_{q}^2$ are fixed given a query, $x_{e}x_{q}+y_{e}y_{q}$ is the inner product similarity we need, while $x_{e}^2,y_{e}^2$ make the equation not monotonic, and we need to look up the hit sphere coordinate at runtime which is expensive. To eliminate them, following the distance calculation mechanics using hit time $t$, we can replace the original entry sphere with a new sphere with identical location but a new radius $R^{'}=\sqrt{R^2+x_{e}^2+y_{e}^2}$, the hit time $t$ becomes
% \begin{equation}
% \label{eq:mips2}
% \begin{aligned}
%     &1-\sqrt{(R^{'})^2-d^2}\\=&1-\sqrt{R^2+x_{e}^2+y_{e}^2-((x_{e}-x_{q})^2+(y_{e}-y_{q})^2)}\\
%     =&1-\sqrt{R^2-x_{q}^2-y_{q}^2+2(x_{e}x_{q}+y_{e}y_{q})}
% \end{aligned}
% \end{equation}
% Now inner product can be directly calculated by pre-defined data without any sphere coordinate looking up. In practice, we do not need to change anything in offline and online process except for adjusting the radius of spheres from $R$ to $\sqrt{R^2+x_{e}^2+y_{e}^2}$. Notice that we steill need to change metric of the cluster in \emph{filtering} from L2 to IP.

% % \subsection{\proj{} Overview and End-to-End Searching Pipeline}


==> optimization.tex <==
\section{Optimizations and Tradeoffs}
\label{sec:Optimizations}
\subsection{Radius-Accuracy Tradeoff}

\subsection{Query as Ray/Primitive}

\subsection{General Optimizations}
\begin{itemize}
    \item Ray packing and reordering.
    \item BVH pre-building.
    \item Pipelining.
\end{itemize}


==> overview.tex <==
\section{\proj{} Search Pipeline and Implementation}
In this section, we will introduce the detail implementation of \proj{} search pipeline with threshold based selective \emph{L2-LUT construction}, together with some challenges and optimizations. 
\subsection{\proj{} End-to-end Search Pipeline}
\begin{figure}[t]
    \centering
      \includegraphics[width=0.99\linewidth]{JUNOOverview.pdf}
    \caption{Overview design of \proj{}, red parts are different from typical \texttt{IVFPQ} process.}
    \label{fig-Overview} 
\end{figure}
Now we describe the end to end searching pipeline of \proj{}, also shown in \Fig{fig-Overview}. 
We first prepare the traversable scene and inverted indices from codebook entries to search points in every subspace offline (line 2 of \Alg{Algo-e2e}). Once a batch of queries arrive, we first conduct an identical filtering like \texttt{IVFPQ} (line 5-7 of \Alg{Algo-e2e}), then we use the RT core to do threshold based selective L2-LUT construction to obtain every query the L2-LUT containing only the entries fall inside the interested region of query projection in every subspace (line 8-9 of \Alg{Algo-e2e}). Finally we lookup the inverted indices with the entries in L2-LUT$[q][c][d]$ for every selected cluster in every subspace (line 11-15 of \Alg{Algo-e2e}), and accumulate the distance of search points belong to $Map[c][d][entry]$ in every subspace (line 16-17 of \Alg{Algo-e2e}). We implement a per query radix sort to return top-k results from all interested search points.
\begin{algorithm}[b]
	\caption{\proj{} end to end search pipeline.}
	\label{Algo-e2e}
    \textbf{Input:} $points[N][D]$, $queries[Q][D]$\\
    \textbf{Input:} $K$, $M=2$, $E$, $C$, $nprobs$\\
    \textbf{Output:} $neighbours\lbrack Q\rbrack\lbrack K\rbrack$
	\begin{algorithmic}[1]
		\Function {JUNO}{$points$, $queries$, $K$, $M$, $E$, $C$, $Q$, $nprobs$}
        \State{$I\leftarrow BuildRTScene(points, M, E, C, r)$}
        \State{$q\_select\_clusters\lbrack Q\rbrack\leftarrow\lbrack~\rbrack$}
        \State{\textbf{// Filtering}}
        \For{ $q$\textbf{ in }$queries$}
            \State{$I.centroids.sort(\lambda~x:L2(x,q)/IP(x,q))$}
            \State{$q\_select\_clusters[q]\leftarrow centroids[0:nprobs]$}
        \EndFor
        \State{\textbf{// Threshold based selective L2-LUT construction}}
        \State{$LUT\leftarrow L2\_LUT(queries,I,q\_select\_clusters)$}
        \State{\textbf{// Distance calculation of interested search points}}
        \For{$q$\textbf{ in }$queries$}
            \State{$result[q]\leftarrow \lbrace id: tot\_d\rbrace$}
            \For{$c\in[0,nprobs), s\in[0,\frac{D}{M})$}
                \State{$item\leftarrow LUT[q][c][s]$}
                \State{$e, d\leftarrow item.entry, item.distance$}
                \For{$p$\textbf{ in }$result[q]$}
                    \State{$p.tot\_d$ += $p.id\in Map[c][s][e]?:d:1.0$}
                \EndFor
            \EndFor
        \EndFor
        \State{\textbf{return }$result[q].sort(\lambda~x:x[1])[0:K]$}
		\EndFunction
	\end{algorithmic}
\end{algorithm}

\subsection{Implementation Challenges}
In this subsection, we introduce several critical implementation details related to the RT core, that will significantly impact the overall performance. 
\paragraph{Efficient Distance Calculation and Dynamic Threshold.}

\begin{figure}[t]
    \centering
      \includegraphics[width=0.99\linewidth]{CalcDistDynR.pdf}
    \caption{We can use the hit time of the ray to (left) calculate the hit distance between query projection and hit entry, (right) dynamically adjust the radius of the sphere a ray can hit by adjusting rays' max time to travel. }
    \label{fig-CalcDistDynR} 
\end{figure}
Notice that in online part of our RT core mapping, we need to i) support dynamic threshold provided as a hyper-parameter by users and ii) calculate exact hit distance between rays of query projections and spheres of codebook entries in all subspaces once hit events occur. Naively, the first requires we change the radius of spheres at runtime, and the second requires we maintain a mapping from sphere id to its coordinate and look-up at runtime. They both have unacceptable overhead. 
While through the time configurations of rays, in specific, maximal travel time $t_{max}$ and hit time $t_{hit}$, we can avoid these overhead. 

For exact hit distance calculation, we can use the hit time reported by the RT core, with the radius of hit sphere we can rapidly calculate the distance from hit point to the center of sphere, which represents the exact distance between the query projection and the codebook entry, as shown in the left part of \Fig{fig-CalcDistDynR}.

For dynamic radius, we can set a smaller $t_{max}$, with which the ray can only hit a smaller region of the sphere as shown in the right part of \Fig{fig-CalcDistDynR}. For example, a $t_{max}=0.64$ means a scaling factor to be $0.8$ when the original threshold is $0.6$.

Notice we raly on the radius of hit spheres, which can be calculated by the region density the query projection falls into with a cheap polynomial regressor inference. 
\paragraph{Supporting Inner Product Similarity.}
Inner product similarity is widely used in image and word embedding. With some transformation, our methodology can support maximal inner product similarity (MIPS) with almost no cost. Recall that if a query ray hit an entry with radius $R$ at distance $d$ and hit time $t$, we have following relation:
\begin{equation}
\label{eq:mips1}
\begin{aligned}
    =&1-\sqrt{R^2-d^2}\\=&1-\sqrt{R^2-((x_{e}-x_{q})^2+(y_{e}-y_{q})^2)}\\
    =&1-\sqrt{R^2-x_{e}^2-y_{e}^2-x_{q}^2-y_{q}^2+2(x_{e}x_{q}+y_{e}y_{q})}
\end{aligned}
\end{equation}
In \Equ{eq:mips1}, $R^2$ and $x_{q}^2,y_{q}^2$ are fixed given a query, $x_{e}x_{q}+y_{e}y_{q}$ is the inner product similarity we need, while $x_{e}^2,y_{e}^2$ make the equation not monotonic, and we need to look up the hit sphere coordinate at runtime which is expensive. To eliminate them, following the distance calculation mechanics using hit time $t$, we can replace the original entry sphere with a new sphere with identical location but a new radius $R^{'}=\sqrt{R^2+x_{e}^2+y_{e}^2}$, the hit time $t$ becomes
\begin{equation}
\label{eq:mips2}
\begin{aligned}
    &1-\sqrt{(R^{'})^2-d^2}\\=&1-\sqrt{R^2+x_{e}^2+y_{e}^2-((x_{e}-x_{q})^2+(y_{e}-y_{q})^2)}\\
    =&1-\sqrt{R^2-x_{q}^2-y_{q}^2+2(x_{e}x_{q}+y_{e}y_{q})}
\end{aligned}
\end{equation}
Now inner product can be directly calculated by pre-defined data without any sphere coordinate looking up. In practice, we do not need to change anything in offline and online process except for adjusting the radius of spheres from $R$ to $\sqrt{R^2+x_{e}^2+y_{e}^2}$. Notice that we steill need to change metric of the cluster in \emph{filtering} from L2 to IP.

\paragraph{Effective Hardware Pipelining.}

\begin{figure}[t]
    \centering
      \includegraphics[width=0.49\linewidth]{Pipeline.pdf}
      \includegraphics[width=0.49\linewidth]{CntL2Rel.pdf}
    \caption{(a) Execution latency breakdown of three stages. (b) Relation between hit count and exact distance of query and search points.}
    \label{fig-PipelineAndCounter} 
\end{figure}
NVIDIA GPUs newer than Ampere architecture support co-running of Tensor core, RT core and CUDA core~\cite{Ampere}. However, naive co-running results in severe interference and slow-down as shown in \Fig{fig-PipelineAndCounter}(a). To enable hardware pipelining, we first map the accumulation in \emph{distance calculation} to the Tensor core. We first organize the interested search points' distance in every subspace into rows and get matrix $A$ with shape $M,K=Q\times sizeof(interested~points)\times nprobs, D/M$ (for simplicity we do some padding for $sizeof(interested~points)$). Then we create a matrix $B$ with shape $K,N=D/M,1$ and set all elements of matrix $B$ to $1.0$. Thus, the accumulation can be done by calculating $A\times B$ and we call \texttt{cublas} API to conduct this matrice multiplication using Tensor core. Then we use CUDA MPS~\cite{MPS} to partition the SM resources into 9:1 for \emph{L2-LUT construction} (uses RT core) and \emph{distance calculation} (uses Tensor core) respectively, notice that 9:1 is a partition with which two stages have similar latency. NVIDIA MIG~\cite{MIG} is an alternative in addition to MPS. With some overhead for data formating, we can now pipeline these two stages. Notice there is a overhead of less than 5\% of latency of \emph{L2-LUT construction} to organize the data from \emph{L2-LUT construction} into matrices format used in \emph{distance calculation}.

For \emph{filtering}, L2 distance can be calculated with $\lVert x-q\rVert_{2}^{2}=\bm{x^{2}}-2xq+\bm{q^{2}}$, where $\bm{x^2}\leftarrow\sum_{i=0}^{D-1}x_{i}^{2}$ is calculated ahead of time. We just calculate the $\bm{q^2}\leftarrow \sum_{i=0}^{D-1}q_{i}^{2}$ for every query. To calculate $2xq$, we use \texttt{cublas} and Tensor core too with $\alpha=-2,\beta=1,A=x, B=q^{T}, C=\bm{x^{2}}(\bm{q^{2}})^{T}$. Inner product is even simpler by calling a \texttt{matmul} with $A=x,B=q^{T}$.

\subsection{Hit Counter Based Selecting}
Currently we still need to conduct several floating operation in \emph{L2-LUT construction} to calculate the radius of a hit sphere and hit distance of a ray. A straightforward idea is to only record hit/miss result with one bit and collect the hit count, supporting by the finding of previous work~\cite{NNHighDim}. So, we study the relation between hit count and exact distance with all spheres are set the radius as the threshold to contain all top-100 search points. As shown in \Fig{fig-PipelineAndCounter}(b), there is strong correlation between these two factors. Given this finding, we implement a hit count-based method since higher hit count implies being close to the query projection in more subspaces.
While there exists false positive and false negative since there can be points being extremely far away from the query projection in few subspaces but close in most of subspaces, makes the total distance huge. So, we introduce a finer-grained hit count-based method with panelty, by adding a sphere with half of the radius for every original sphere. The hit count will be +1 only if the ray hit the inner sphere, and will be -1 if the ray miss two spheres as a panelty. As shown by the blue points in \Fig{fig-PipelineAndCounter}(b), the relation between hit count and exact distance is stronger, with less false positive and false negative. But notice that there always exist false positive/negative since original distance data are collapsed into limited hit count. 
hit count-based selecting require none floating point operation in hit shader, and we have another trade-off between QPS and search quality. 

==> post_revision_cover_letter.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\label{CoverLetter}
\thispagestyle{empty}
\addtocounter{page}{-1}
\begin{table}[t]
    \centering
    \begin{tabular}{@{}c|p{7.5cm}|p{6cm}@{}}
    % \toprule
    \multicolumn{3}{c}{\textbf{\huge Post Revision Comment Cover Letter}} \\
    \multicolumn{3}{c}{\textcolor{red}{\emph{*click IDs in the cover letter to jump to the content, and click the IDs in the contents to jump back to this page.}}}                                                                                                                                                        \\ \midrule
    \textbf{ID}                        & \begin{tabular}[c]{@{}c@{}}Comments\end{tabular} & \begin{tabular}[c]{@{}c@{}}Actions\end{tabular}                                                                                                                                                                                            \\ \midrule
    \multicolumn{3}{c}{\textbf{Post Revision Comments}}                                                                                                                                                                                                                                                                                                                                          \\ \midrule
    \multicolumn{1}{c|}{\hyperref[fig-Example]{\textbf{PR-A}}} & Section 2: The new sentence needs attention "Notices there are other indexing and encoding techniques, and we detailed discuss them in Sec.7."                                      & We tweak this sentence in Section 2.\\ \midrule
    \multicolumn{1}{c|}{\hyperref[PR-B]{\textbf{PR-B}}} & Evaluation: Consider a shade of gray that allows the reader to see the point even when the paper is printed.                                      & We adjust this figure by shading the points in this figure.\\ \midrule
    \multicolumn{1}{c|}{\hyperref[PR-C]{\textbf{PR-C}}} & Unclear what benefit the last paragraph in Sec 6.5 brings to the current paper.                                      & We clarify the purpose of the newly added paragraph and corresponding figure.\\ \midrule
    \multicolumn{1}{c|}{\hyperref[PR-D]{\textbf{PR-D}}} & Indicate the limitation of the current implementation regarding the GPU memory for Billion+ datasets.                                      & We add the clarification in evaluation setup.\\ \midrule
        
\end{tabular}
    \end{table}

==> revision_cover_letter.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\label{CoverLetter}
\thispagestyle{empty}
\addtocounter{page}{-1}
\begin{table}[b]
    \centering
    \begin{tabular}{@{}ccccp{11cm}@{}}
    % \toprule
    \multicolumn{5}{c}{\textbf{\huge Revision Cover Letter}} \\
    \multicolumn{5}{c}{\textcolor{blue}{\emph{*click IDs in the cover letter to jump to the content, and click the IDs in the contents to jump back to the cover letter.}}}                                                                                                                                                        \\ \midrule
    \textbf{ID}                        & \begin{tabular}[c]{@{}c@{}}Related\\ Action(s)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Accept\\ Condition(s)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Page(s)\\ No.\end{tabular} & Descriptions                                                                                                                                                                                            \\ \midrule
    \multicolumn{5}{c}{\textbf{Feedback from reviewers and authors' corresponding actions}}                                                                                                                                                                                                                                                                                                                                          \\ \midrule
    \multicolumn{1}{c|}{\hyperref[R-A]{\textbf{R-A}}} & \multicolumn{1}{c|}{5}                                      & \multicolumn{1}{c|}{3}                                        & \multicolumn{1}{c|}{3}                                & We clarify the corresponding description of the third step of the \texttt{PQ} in Fig 2.                                                                                                    \\ \midrule
    \multicolumn{1}{c|}{\hyperref[fig-RTPipe]{\textbf{R-B}}}  & \multicolumn{1}{c|}{5}                                      & \multicolumn{1}{c|}{3}                                        & \multicolumn{1}{c|}{3}                                & We add the detailed desciption of BVH and AABB algorithm.                                                                                                                          \\ \midrule
    \multicolumn{1}{c|}{\hyperref[R-C]{\textbf{R-C}}} & \multicolumn{1}{c|}{1,3,6}                                  & \multicolumn{1}{c|}{1,a,3}                                    & \multicolumn{1}{c|}{10}                               & We add R100@1000 result of SIFT1M, DEEP1M, and TTI1M. We also add R1@100 result of DEEP100M (an extra 100M dataset we have added). Finally, we adjust the description of Pareto Frontier in \Fig{fig-recallres}. \\ \midrule
    \multicolumn{1}{c|}{\hyperref[R-D]{\textbf{R-D}}} & \multicolumn{1}{c|}{6}                                      & \multicolumn{1}{c|}{a}                                        & \multicolumn{1}{c|}{10}                               & We add the configurations of 100M datasets and optimize the presentation.                                                                                                          \\ \midrule
    \multicolumn{1}{c|}{\hyperref[R-E]{\textbf{R-E}}} & \multicolumn{1}{c|}{2,7,8}                                  & \multicolumn{1}{c|}{2,b}                                      & \multicolumn{1}{c|}{10}                               & We add stronger baseline \texttt{HNSW} to all datasets and update the description of baseline configurations.                                                                               \\ \midrule
    \multicolumn{1}{c|}{\hyperref[R-F]{\textbf{R-F}}} & \multicolumn{1}{c|}{1}                                      & \multicolumn{1}{c|}{1}                                        & \multicolumn{1}{c|}{10}                               & We add the description of R100@1000 metric.                                                                                                                                        \\ \midrule
    \multicolumn{1}{c|}{\hyperref[R-G]{\textbf{R-G}}} & \multicolumn{1}{c|}{2}                                      & \multicolumn{1}{c|}{2}                                        & \multicolumn{1}{c|}{10}                               & We optimize the descriptions of three configurations of JUNO.                                                                                                                      \\ \midrule
    \multicolumn{1}{c|}{\hyperref[R-H]{\textbf{R-H}}} & \multicolumn{1}{c|}{7,8}                                    & \multicolumn{1}{c|}{2,b}                                      & \multicolumn{1}{c|}{10}                               & We evaluate the baseline with stronger configuration \texttt{HNSW} on all datasets, together with the best performed \texttt{PQ} configurations.                           \\ \midrule
    \multicolumn{1}{c|}{\hyperref[R-I]{\textbf{R-I}}} & \multicolumn{1}{c|}{9}                                      & \multicolumn{1}{c|}{b}                                        & \multicolumn{1}{c|}{10,11}                            & We evaluate the performance of the baseline with various configurations and provide corresponding justifications on \texttt{PQ} selection and whether to enable \texttt{HNSW}.                       \\ \midrule
    \multicolumn{1}{c|}{\hyperref[R-J]{\textbf{R-J}}} & \multicolumn{1}{c|}{6}                                      & \multicolumn{1}{c|}{a}                                        & \multicolumn{1}{c|}{11}                               & We report the performance improvement on two 100M datasets, one is the original (SIFT100M) and the other is added by us (DEEP100M).                                                \\ \midrule
    \multicolumn{1}{c|}{\hyperref[R-K]{\textbf{R-K}}} & \multicolumn{1}{c|}{1,4}                                    & \multicolumn{1}{c|}{1,3}                                      & \multicolumn{1}{c|}{11}                               & We report the results in both R1@100 and R100@1000 metrics, we also discuss the neighbor quality in R1@100 metric, which is R100@100 as mentioned in our rebuttal response.        \\ \midrule
    \multicolumn{1}{c|}{\hyperref[R-L]{\textbf{R-L}}} & \multicolumn{1}{c|}{10}                                     & \multicolumn{1}{c|}{2,b,3}                                      & \multicolumn{1}{c|}{12}                               & We clarify the static radius configuration in effectiveness analysis of \Fig{fig-breakdown}b.                                                                                                              \\ \midrule
    \multicolumn{1}{c|}{\hyperref[R-M]{\textbf{R-M}}} & \multicolumn{1}{c|}{11}                                     & \multicolumn{1}{c|}{2,b,3}                                      & \multicolumn{1}{c|}{12}                               & We clarify the configuration and meaning of hardware sensitivity analysis of \Fig{fig-sensitivity}a.                                                             \\ \midrule
    \multicolumn{1}{c|}{\hyperref[R-N]{\textbf{R-N}}} & \multicolumn{1}{c|}{12}                                     & \multicolumn{1}{c|}{2,b,3}                                      & \multicolumn{1}{c|}{11,12}                               & We clarify the meaning of our effectiveness and sensitivity analysis in text.                                                                                               \\ \midrule
    \multicolumn{5}{c}{\textbf{Other revision actions taken by authors}}                                                                                                                                                                                                                                                                                                                                                                    \\ \midrule
    \multicolumn{1}{c|}{\hyperref[R-O]{\textbf{R-O}}} & \multicolumn{1}{c|}{/}                                      & \multicolumn{1}{c|}{3}                                        & \multicolumn{1}{c|}{2,13}                               & We add some detailed descriptions on graph based index.                                                                                                                            \\ \midrule
    \multicolumn{1}{c|}{\hyperref[R-P]{\textbf{R-P}}} & \multicolumn{1}{c|}{/}                                      & \multicolumn{1}{c|}{3}                                        & \multicolumn{1}{c|}{13}                            & We add some clarification about capability of \proj{}, in response to rebuttal question A1.                                                                       \\ \midrule
    \multicolumn{1}{c|}{\hyperref[fig-Example]{\textbf{R-Q}}} & \multicolumn{1}{c|}{/}                                      & \multicolumn{1}{c|}{3}                                        & \multicolumn{1}{c|}{2}                                & We add some clarification about the novelty and contributions of \proj{}, in response to rebuttal question Common1.                                                                   \\ \bottomrule
    \multicolumn{1}{c|}{\hyperref[R-R]{\textbf{R-R}}} & \multicolumn{1}{c|}{/}                                      & \multicolumn{1}{c|}{3}                                        & \multicolumn{1}{c|}{12,13}                                & We add some discussion on accuracy guarantee and nature of dataset reviewers may concern, in response to rebuttal question A2 and Common3                                                                  \\ \bottomrule
    \multicolumn{1}{c|}{\hyperref[fig-Overview]{\textbf{R-S}}} & \multicolumn{1}{c|}{/}                                      & \multicolumn{1}{c|}{3}                                        & \multicolumn{1}{c|}{7}                                & We optimize the presentation and equation in inner-product metric support.                                                                 \\ \bottomrule
    \end{tabular}
    \end{table}
